The Schr\"odinger Bridge between Gaussian Measures has a Closed Form

The static optimal transport $(\mathrm{OT})$ problem between Gaussians seeks to recover an optimal map, or more generally a coupling, to morph a Gaussian into another. It has been well studied and applied to a wide variety of tasks. Here we focus on the dynamic formulation of OT, also known as the Schr\"odinger bridge (SB) problem, which has recently seen a surge of interest in machine learning due to its connections with diffusion-based generative models. In contrast to the static setting, much less is known about the dynamic setting, even for Gaussian distributions. In this paper, we provide closed-form expressions for SBs between Gaussian measures. In contrast to the static Gaussian OT problem, which can be simply reduced to studying convex programs, our framework for solving SBs requires significantly more involved tools such as Riemannian geometry and generator theory. Notably, we establish that the solutions of SBs between Gaussian measures are themselves Gaussian processes with explicit mean and covariance kernels, and thus are readily amenable for many downstream applications such as generative modeling or interpolation. To demonstrate the utility, we devise a new method for modeling the evolution of single-cell genomics data and report significantly improved numerical stability compared to existing SB-based approaches.

==> content/background.tex <==
\newmacro{\tdriftbase}{ f }
%\newcommand{\tdrift}[1][\ctime]{ \tdriftbase\parens*{ #1 } }

\NewDocumentCommand{\tdrift}{ O{\ctime} O{\refsde} }{ \tdriftbase\parens*{#1,#2} }

\newmacro{\SB}{ {\scriptscriptstyle\textup{SB}} } %{\scriptscriptstyle\mathrm{SB}} }

\newcommand{\pSB}[1]{  p^{\SB}_{#1} }

%It can be shown that \eqref{eq:StaticGaussianSB} is \eqref{eq:GaussianSB} restricted to the initial and final marginals \citep{leonard2013survey,chen2021stochastic}.

%\newmacro{\pdata}{ \mathbb{P}_{\mathrm{data}} }
%
%\newmacro{\psimple}{ \mathbb{P}_{\mathrm{simple}} }


%\para{\acl{SB}}
%The intuition behind the \ac{SB} is best illustrated by the simple case where $\refpro = \Wiener$, which presupposes that the process $\Pmargin$ we wish to reconstruct behaves as a physical system in thermal equilibrium. By the Gaussian increments of $\Wiener$, for any marginal $\distinit$ at time $0$, $\Wiener$ would predict the distribution at time $\horizon$ to be $\distinit \ast  \Ncal(0,\horizon\cdot\eye)$ where $\ast$ denotes the convolution operator. If this distribution differs from the actual data $\distend$, then $\Pmargin$ must also differ from $\Wiener$. To find out $\Pmargin$, \citet{schrodinger1931umkehrung,schrodinger1932theorie} considers the objective \eqref{eq:SB} as the ``mostly likely process'' that explains the marginal distributions $\distinit,\distend$ relative to $\Wiener$. This idea generalizes verbatim to any reference process $\refpro$.
% he objective \eqref{eq:SB} 
% it means that $\Pmargin$  
% In the simplest scenario where $\refpro = \sdev\Wiener$, the system \eqref{eq:SB} becomes the what \citet{schrodinger1931umkehrung,schrodinger1932theorie} considers as a ``diffusion'' model for the quantum phenomena of electrons: Before any measurement is taken, the electrons diffuse in a thermal equilibrium state and hence behave like \aclp{BM}. After measurements, the electrons collapse to deterministic ``particles'' and no longer behave in a stochastic manner.

% in \eqref{eq:SB}. Th

% Consider the objective \eqref{eq:SB} when $\refpro = \sdev\Wiener$ is simply the \acl{BM}. 
% Given two marginal distributions $\distinit, \distend$, the \emph{\ac{SB}} is an entropy minimization problem of the form:
% \begin{equation}
% \label{eq:generalSB}
% %\tag{SB}
% \min_{ \Pinit = \distinit,\; \Pend = \distend} \KL{\Pmargin}{\refpro}
% \end{equation}
% where $\refpro$ is a ``reference'' stochastic process that needs to be chosen beforehand. 

\vspace{-6pt}
%In this section, we recollect certain useful facts regarding \ac{SB}.% that are useful throughout the rest of the paper.
\textbf{Review of \ac{SB}.}
In principle, one can take the reference process $\refpro$ in \eqref{eq:SB-updated} to be any \ac{SDE} of the form:% with drift and scale,
\begin{align}
\label{eq:general-refsde}
\drefsde  = \tdrift  \dt + \volat \dWiener[\ctime]\equiv \tdriftbase \dt + \volatbase \dWiener[\ctime]
\end{align}
with some initial condition $\refsdebase_0$. In this case, %When $\refpro = \sdev\Wiener$, \eqref{eq:generalSB} reduces to the classical \eqref{eq:SB}.
%An important fact is that $\refpro$ enters the optimality condition of \eqref{eq:generalSB} only through the \emph{conditional} distributions of the form $\left.\refsde \right\vert \refsde[0], \refsde[\horizon]$ \citep{leonard2013survey}. %, we will ignore the initial condition for $\refsde$.
~it turns out that the solution to \eqref{eq:SB-updated} is itself given by two coupled \acp{SDE} of the form \citep{leonard2013survey}
\begin{subequations}
\begin{eqnarray}
\label{eq:SB-sde-forward}
\dsde &= \parens*{\tdriftbase +  \volatbase \SBfbase_\ctime} \dt + \volatbase \dWiener[\ctime],\; \sde[0] \sim \distinit, \\%\; & \sde[0] \sim \Pinit, \\
\label{eq:SB-sde-backward}
\dsde &= \parens{\tdriftbase -  \volatbase \SBbbase_\ctime} \dt + \volatbase \dWiener[\ctime],\; \sde[\horizon] \sim \distend,%\; & \sde[\horizon] \sim \Pend.
\end{eqnarray}
\end{subequations}
where $\SBfbase_\ctime, \SBbbase_\ctime \from \R^\vdim \to \R^\vdim$ are two time-indexed smooth \emph{vector fields} called the optimal forward and backward drift, respectively, and \eqref{eq:SB-sde-backward} runs backward in time (\ie from $\horizon \to 0$). %and satisfies many interesting properties \citep{nelson1967dynamical,leonard2013survey,chen2021stochastic}.
~If we parametrize the forward drift by $\SBf$ and the backward drift by $\SBb$ with some parameters $\paramf,\paramb$, then the negative likelihood function for $\paramf$ and $\paramb$ can be expressed as \citep{chen2021likelihood}
\begin{subequations}
\begin{align}
\lossb =  \int_0^\horizon \mathbb{E}_{\eqref{eq:SB-sde-forward}}\Big[ \frac{1}{2}\norm{\SBbbase^{\paramb}_\ctime}^2 &+\volatbase \Div \SBbbase^{\paramb}_\ctime+ \inner{\SBfbase^{\paramf}_\ctime}{\SBbbase^{\paramb}_\ctime} \dt \Big\vert \sde[0] = \point_0 \Big] ,  \\
\lossf =  \int_0^\horizon \mathbb{E}_{\eqref{eq:SB-sde-backward}}\Big[ \frac{1}{2}\norm{\SBfbase^{\paramf}_\ctime}^2 &+\volatbase \Div \SBfbase^{\paramf}_\ctime + \inner{\SBbbase^{\paramb}_\ctime}{\SBfbase^{\paramf}_\ctime} \dt \Big\vert \sde[\horizon] = \point_{\horizon} \Big],
\end{align}
\end{subequations}
where $\Div$ denotes the divergence operator w.r.t. the $\point$ variable: For any $v\from \R^\vdim \to \R^\vdim$, $\Div v(\point) \defeq \sum_{\coord=1}^{\vdim} \ddc v_\coord(\point)$.

%\textbf{\acp{SGM} and pretraining of \eqref{eq:SB}.\,\,}
% The generative modeling problem corresponds to the setting when $\distend = \Ncal(0,\eye)$. In this case, the celebrated \ac{SGM}, in its \ac{SDE} formulation \citep{song2020score}, can be interpreted as approximating \eqref{eq:SB-sde-forward}-\eqref{eq:SB-sde-backward} by choosing an appropriate $\drefsde$ in \eqref{eq:general-refsde} such that $\refsde[\horizon] \simeq \Ncal(0,\eye)$ for any initial condition $\refsde[0]$, which then implies that $\SBfbase_\ctime\simeq 0$ and \eqref{eq:SB-sde-forward} coincides with \eqref{eq:general-refsde}. Thus, solving \eqref{eq:generalSB} reduces to learning only the backward drift $\SBbbase_\ctime$; see \citep{chen2021likelihood} for details.
%\para{Pre-training of \eqref{eq:generalSB}}
%\looseness -1 
\textbf{Pretraining of \ac{SB}.}
Evaluating the negative likelihood $\lossb$ involves simulating the \ac{SDE} \eqref{eq:SB-sde-forward} with a general drift function $\SBf$, which is an expensive operation even for simple reference \acp{SDE} $\refsde$ such as Brownian motions. However, if $\SBfbase_\ctime \equiv 0$, then the \emph{conditional distribution} $\sde \vert \sde[0] = \point_0$ of \eqref{eq:SB-sde-forward} often admits a closed-form expression since it merely simulates $\refsde$. For this reason, previous work on solving \eqref{eq:SB-updated} \citep{chen2021likelihood, de2021diffusion, vargas2021solving} propose to initialize $\paramf_0$ such that $\SBf[\ctime][\cdot][\paramf_0] \equiv 0$ (for instance, $\SBf[\ctime][\cdot][\paramf_0]$ being a neural network with zero output weights), and train the backward drift $\SBb$ first. This is called \emph{pretraining} in the literature, and has proved to be of central importance in the empirical performance of \ac{SB} for generative modeling. In our experiments, we continue to observe the substantial benefit of pretraining when both $\distinit$ and $\distend$ are complicated distributions.

% \citep{vargas2021solving}\citep{de2021diffusion}
